Self-supervised learning for audio-visual speaker diarization

Speaker diarization, which is to find the speech segments of specific speakers, has been widely used in human-centered applications such as video conferences or human-computer interaction systems. In this paper, we propose a self-supervised audio-video synchronization learning method to address the problem of speaker diarization without massive labeling effort. We improve the previous approaches by introducing two new loss functions: the dynamic triplet loss and the multinomial loss. We test them on a real-world human-computer interaction system and the results show our best model yields a remarkable gain of +8%F1-scoresas well as diarization error rate reduction. Finally, we introduce a new large scale audio-video corpus designed to fill the vacancy of audio-video datasets in Chinese.

==> comment.tex <==
1. 增加第一种metric的说明
2. curve different window
3. 增加f score
4. 公式修改
done 5. 帧的排列 figure3gt下面
done 6. github website link放入文章
done 7. network
